Co-synthesis of Histopathology Nuclei Image-Label Pairs using a Context-Conditioned Joint Diffusion Model

In multi-class histopathology nuclei analysis tasks, the lack of training data becomes a main bottleneck for the performance of learning-based methods. To tackle this challenge, previous methods have utilized generative models to increase data by generating synthetic samples. However, existing methods often overlook the importance of considering the context of biological tissues (e.g., shape, spatial layout, and tissue type) in the synthetic data. Moreover, while generative models have shown superior performance in synthesizing realistic histopathology images, none of the existing methods are capable of producing image-label pairs at the same time. In this paper, we introduce a novel framework for co-synthesizing histopathology nuclei images and paired semantic labels using a context-conditioned joint diffusion model. We propose conditioning of a diffusion model using nucleus centroid layouts with structure-related text prompts to incorporate spatial and structural context information into the generation targets. Moreover, we enhance the granularity of our synthesized semantic labels by generating instance-wise nuclei labels using distance maps synthesized concurrently in conjunction with the images and semantic labels. We demonstrate the effectiveness of our framework in generating high-quality samples on multi-institutional, multi-organ, and multi-modality datasets. Our synthetic data consistently outperforms existing augmentation methods in the downstream tasks of nuclei segmentation and classification.

==> _.tex <==
\appendix
\begin{center}
    \addcontentsline{toc}{chapter}{Appendix}
    \LARGE \textbf{Appendix}
\end{center}

this is Supplementary Material.

\section*{Appendix A. Color Quality}
\label{sec:color}

\begin{figure}[htb!]
    \centering
    \includegraphics[width=\textwidth, keepaspectratio]{figures/suppl_color_v6.pdf}
    \caption{
    Color quality comparison of synthetic images on PanNuke across different tissue types. Ours produced images with the appropriate color distribution for each tissue type, whereas SDM synthesized images exhibited unrealistic colors.
    }
    \label{fig:color_comp}
\end{figure}




\begin{table}[]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Pathologist evaluation: additional comments}
    \label{tab:path_eval_comments}
\end{table}


\section*{Appendix B. Survey Detail}

\section*{Appendix C. Additional Results}

\section*{Appendix D. Ablation Studies}


==> tables/downstream_cls.tex <==
% \begin{table}[htb]
%   \caption{
%   Downstream task (segmentation and classification) performance comparison dataset using Hover-Net~\cite{graham2019hover} as a baseline network.
%   }
%   \label{tab:downstream}
%   \centering
%   \begin{tabular}{@{}lll@{}}
%     \toprule
%     Heading level & Example & Font size and style\\
%     \midrule
%     Title (centered)  & {\Large\bf Lecture Notes \dots} & 14 point, bold\\
%     1st-level heading & {\large\bf 1 Introduction} & 12 point, bold\\
%     2nd-level heading & {\bf 2.1 Printing Area} & 10 point, bold\\
%     3rd-level heading & {\bf Headings.} Text follows \dots & 10 point, bold\\
%     4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
%     4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
%     4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
%     4th-level heading & {\it Remark.} Text follows \dots & 10 point, italic\\
%   \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[htb!]
\caption{
Downstream task (classification) performance comparison using Hover-Net~\cite{graham2019hover} as a baseline network.
The best results are in \textbf{bold} and the second best are \underline{underlined}.
}% Here, Ours refers to Ours + $hv$.}
\label{tab:downstream}
\centering
\renewcommand{\arraystretch}{1.05}
\renewcommand{\tabcolsep}{5.2pt}
\begin{tabular}{l
>{\small}l
|>{\small}c
>{\small}c
>{\small}c
>{\small}c
>{\small}c
>{\small}c
>{\small}c
}
% l|ccccc|ccccccc}
\toprule\specialrule{0.05pt}{0pt}{0pt}
% &\specialrule{0.2pt}{0pt}{0pt}
% \cline{2-13}
\textbf{Dataset} &  \textbf{Method} & $F_{d}$ & $F^{c_1}$ & $F^{c_2}$ & $F^{c_3}$ & $F^{c_4}$ & $F^{c_5}$ & $F^{c_6}$
\\ 
\hline\hline
%           & Base  & 0.798 & 0.475 & 0.420 & 0.169 & 0.434 & 0.557 & - \\
%  Lizard   & Base + Aug. & 0.813 & 0.492& 0.449& 0.160 & 0.472 & 0.602 & - \\ 
% % \hline\hline
%           & Base + Ours & 0.815 & 0.508 & 0.461 & 0.169 & 0.472 & 0.614 & - \\
          & Base  & 0.798 & 0.475 & 0.420 & 0.169 & 0.434 & 0.557 & - \\
 Lizard   & Base + Aug. & 0.813 & 0.492& 0.449& 0.160 & 0.472 & 0.602 & - \\ 
% \hline\hline
          & Base + Ours & 0.815 & 0.508 & 0.461 & 0.169 & 0.472 & 0.614 & - \\

\hline
          & Base  & 0.798 & 0.475 & 0.420 & 0.169 & 0.434 & 0.557 & - \\
 PanNuke  & Base + Aug. & 0.813 & 0.492& 0.449& 0.160 & 0.472 & 0.602 & - \\ 
% \hline\hline
          & Base + Ours & 0.815 & 0.508 & 0.461 & 0.169 & 0.472 & 0.614 & - \\
\hline
          & Base  & 0.798 & 0.475 & 0.420 & 0.169 & 0.434 & 0.557 & - \\
 EndoNuke & Base + Aug. & 0.813 & 0.492& 0.449& 0.160 & 0.472 & 0.602 & - \\ 
% \hline\hline
          & Base + Ours & 0.815 & 0.508 & 0.461 & 0.169 & 0.472 & 0.614 & - \\
\hline
%           & Base  & 0.798 & 0.475 & 0.420 & 0.169 & 0.434 & 0.557 & - \\
%  EndoNuke & Base + Aug. & 0.813 & 0.492& 0.449& 0.160 & 0.472 & 0.602 & - \\ 
% % \hline\hline
%           & Base + Ours & 0.815 & 0.508 & 0.461 & 0.169 & 0.472 & 0.614 & - \\
\toprule\specialrule{0.05pt}{0pt}{0pt}
\end{tabular}

\end{table}

% \begin{tabular}{
% >{\small}l|
% >{\small}c
% >{\small}c
% >{\small}c
% >{\small}c
% >{\small}c|
% >{\small}c
% >{\small}c
% >{\small}c
% >{\small}c
% >{\small}c
% >{\small}c
% >{\small}c
% }
% % l|ccccc|ccccccc}
% \toprule
% \specialrule{0.2pt}{0pt}{0pt}
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Segmentation}}  & \multicolumn{7}{c}{\textbf{Classification}}  
% \\
% % \cline{2-13}
% \multicolumn{1}{c|}{} & Dice & AJI & DQ & SQ & PQ & $F_{d}$ & $F^{c_1}$ & $F^{c_2}$ & $F^{c_3}$ & $F^{c_4}$ & $F^{c_5}$ & $F^{c_6}$\\ \hline\hline
% Baseline  & 0.664 & 0.402 &	0.484 & 0.748 & 0.371 &  0.601 & 0.240 & 0.663 & 0.290 & 0.338 & 0.430 & 0.376
% \\
% Baseline + (Ours + $hv$) & 0.698 & 0.453 & 0.550 & 0.761 & 0.428 & 0.652 & 0.289 & 0.701 & 0.337 & 0.390 & 0.453 & 0.440
% \\ 
% \hline\hline
% Baseline + SDM & 0.706 & 0.464 & 0.564 & 0.761 & 0.439 & 0.668 & 0.334 &	0.711 & 0.355 & 0.395 & 0.443 & 0.457 
% \\
% \toprule
% \end{tabular}

% \end{table}

==> tables/mdice.tex <==
\begin{wraptable}{l}{.48\textwidth}
\centering
\vspace{-25pt}
\caption{
    Comparative results of instance separation algorithms, evaluated by mDice.
    The best results are in \textbf{bold} and the second best are \underline{underlined}.
}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{1.2pt}
\label{table:mdice}
\begin{tabular}{
>{\scriptsize}l|
>{\scriptsize}c
>{\scriptsize}c
>{\scriptsize}c
}
\toprule
\specialrule{0.1pt}{0pt}{0pt}
% {\textbf{Method}} & {Lizard} & {PanNuke} & {EndoNuke} \\

\multirow{2}{*}{\textbf{\qwer{Method}}} & \multicolumn{3}{c}{\textbf{\qwer{mDice}}} \\
\multicolumn{1}{c|}{} & {Lizard} & {PanNuke} & {EndoNuke} \\

\hline\hline

Connectivity-based & \underline{{0.9383}} & {0.9146} & {0.5524} \\
 
Yu~\textit{et al.}~\cite{diffaug} & {0.9374} & \underline{{0.9462}} & \underline{{0.9268}} \\
 
\hline

\textbf{Ours} & \textbf{{0.9754}} & \textbf{{0.9980}} & \textbf{{0.9634}} \\

\toprule
\specialrule{0.1pt}{0pt}{0pt}
\end{tabular}


\vspace{-15pt}
\end{wraptable}

==> tables/methods.tex <==
\begin{wraptable}{l}{.61\textwidth}
\centering
\vspace{-33pt}
\caption{Comparative overview of generative models by conditional inputs and output targets.
}
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1.0pt}
\label{table:methods}
\begin{tabular}{
>{\qhrh}l|
>{\qhrh}l|
>{\qhrh}c
>{\qhrh}c
>{\qhrh}c
}
\toprule
\specialrule{0.1pt}{0pt}{0pt}

\multirow{2}{*}{\textbf{\scriptsize{Method}}} & \multirow{2}{*}{\textbf{\scriptsize{Condition}}} & \multicolumn{3}{c}{\textbf{\scriptsize{Generation Target}}}\\


& & {Image} & {Dist.Map} & {Label}\\
\hline\hline

{NuDiff \cite{diffaug}} & {None} &
\checkmark  & \checkmark  & \checkmark \\

{SemanticPalette \cite{semantic-palette}} & {Class Proportion} &
\checkmark  & -  & \checkmark \\

{GCDP \cite{gcdp}} & {Text} &
\checkmark  & -  & \checkmark \\

{SDM \cite{sdm}} & {Label, Instance Edge} &
\checkmark & - & - \\

\hline
{\textbf{Ours}} & {Text, Point Map} &
\checkmark  & \checkmark  & \checkmark \\


\toprule
\specialrule{0.1pt}{0pt}{0pt}
\end{tabular}

\vspace{-15pt}
\end{wraptable}
